Introducing $\gamma$-lifting for Learning Nonlinear Pulse Shaping in Coherent Optical Communication

Pulse shaping for coherent optical fiber communication has been an active area of research for the past decade. Most of the early schemes are based on classic Nyquist pulse shaping that was originally intended for linear channels. The best known classic scheme, the split digital back-propagation (DBP), uses joint pre-distortion and post equalization and hence, a nonlinear transmitter (TX); it, however, suffers from spectral broadening on the fiber due to the Kerr-effect. With the advent of deep learning in communications, it has been realized that an Autoencoder can learn to communicate efficiently over the optical fiber channel, jointly optimizing geometric constellations and pulse shaping - while also taking into account linear and nonlinear impairments such as chromatic dispersion and Kerr-nonlinearity. E.g., arXiv:2006.15027 shows how an Autoencoder can learn to mitigate spectral broadening due to the Kerr-effect using a trainable linear TX. In this paper, we extend this linear architectural template to a scalable nonlinear pulse shaping consisting of a Convolutional Neural Network at both transmitter and receiver. By introducing a novel $\gamma$-lifting training procedure tailored to the nonlinear optical fiber channel, we achieve stable Autoencoder convergence to pulse shapes reaching information rates outperforming the classic split DBP reference at high input powers.

==> usr/content/gamma-lifting/abstract.tex <==
% !TeX spellcheck = en_US
Pulse shaping for coherent optical fiber communication has been an active area of research for the past decade. Most of the early schemes are based on classic Nyquist pulse shaping that was originally intended for linear channels.
The best known classic scheme, the \emph{split \acl{DBP}},
uses joint \acl{PD} and \acl{PE} and hence, a \emph{nonlinear} \acl{TX}; it, however, suffers from spectral broadening on the fiber due to the Kerr-effect.
With the advent of deep learning in communications, it has been realized that an ``\acl{AE}'' can learn to communicate efficiently over the optical fiber channel, jointly optimizing geometric constellations and pulse shaping -- while also taking into account linear and nonlinear impairments such as chromatic dispersion and Kerr-nonlinearity. E.g., \cite{uhlemann_deep-learning_2020} shows how an \acl{AE} can learn to mitigate spectral broadening due to the Kerr-effect using a trainable \emph{linear} \acl{TX}.
In this paper, we extend this \emph{linear} architectural template to a scalable \emph{nonlinear pulse shaping} consisting of a \acl{CNN} at both transmitter and receiver.
By introducing a novel $\gamma$-lifting training procedure tailored to the nonlinear optical fiber channel, we achieve stable \acl{AE} convergence to pulse shapes reaching information rates outperforming the classic split \acl{DBP} reference at high input powers.



==> usr/content/gamma-lifting/content.tex <==
% !TeX spellcheck = en_US
\mode*

\title{Introducing $\gamma$-lifting for Learning Nonlinear\\Pulse Shaping in Coherent Optical Communication}
}

\author{%
	\IEEEauthorblockN{%
		Tim Uhlemann, Alexander Span, Sebastian D\"orner, and Stephan ten Brink\\}%
	\IEEEauthorblockA{%
		\textit{Institute of Telecommunications}\\
		\textit{University of  Stuttgart}\\
		Pfaffenwaldring 47, 70569 Stuttgart, Germany\\
		\{uhlemann,span,doerner,tenbrink\}@inue.uni-stuttgart.de\\
	}	
}

\maketitle

\begin{abstract}
	Motivated by the recent success of end-to-end training of communications in the wireless domain, we strive to adapt the end-to-end-learning idea from the wireless case (i.e., linear) to coherent optical fiber links (i.e., nonlinear). Although, at first glance, it sounds like a straightforward extension, it turns out that several pitfalls exist – in terms of theory but also in terms of practical implementation. This paper analyzes an autoencoder’s potential and limitations for the optical fiber under the influence of Kerr-nonlinearity and chromatic dispersion. As there is no exact capacity limit known and, hence, no analytical perfect system solution available, we set great value to the interpretability on the learnings of the autoencoder. Therefore, we design its architecture to be as close as possible to the structure of a classic communication system, knowing that this may limit its degree of freedom and, thus, its performance. Nevertheless, we were able to achieve an unexpected high gain in terms of spectral efficiency compared to a conventional reference system.
	%The main contribution of this work can be divided into:
	%• To the best of our knowledge, the first joint analysis of Kerr-nonlinearity and chromatic dispersion in an end-to-end learning system
	%• A summary of the major difficulties of autoencoder-based communications for the coherent optical fiber link
	%• Analysis of achievable rate of the proposed system
\end{abstract}

\begin{figure*}[ht] % DBP
	\begin{subfigure}[c]{\textwidth}
		\centering
		\includesvg[width=\textwidth]{system-model}
		\subcaption{}
		\label{fig:system}
		\vspace{0em}
	\end{subfigure}
	\begin{subfigure}[c]{\textwidth}
		\centering
		\includesvg[width=0.9\textwidth, inkscapearea=page]{dbp-tx}
		\subcaption{}
		\label{fig:dbp-tx}
		\vspace{0em}
	\end{subfigure}
	\begin{subfigure}[c]{\textwidth}
		\centering
		\includesvg[width=0.6\textwidth, inkscapearea=page]{dbp-rx}
		\subcaption{}
		\label{fig:dbp-rx}
		\vspace{0em}
	\end{subfigure}
 
	\caption{System model with (\subref{fig:system}) overview that holds for conventional as well as \ac{AE} setup, (\subref{fig:dbp-tx}) the \ac{DSP} for the conventional  \ac{TX}, and (\subref{fig:dbp-rx}) the \ac{RX} based on split \ac{DBP}.}
\end{figure*}

\section{Introduction}

For the design of an optical fiber communication system with high \ac{SE} one requires higher order modulation formats and thus a high \ac{SNR} at the \ac{RX}. This, in turn, needs a high launch power at the \ac{TX}. Furthermore, a \ac{TBP} close to one should be chosen, i.e., symbol rate and occupied bandwidth should almost be the same. This, in general, holds for the copper and wireless (radio frequency) channel. In contrast, for the optical fiber, a high input power results in a large Kerr-nonlinearity and hence, in a highly distorted signal at the \ac{RX} \cite{millar_mitigation_2010}. Apart from the signal-noise interaction, in a single channel scenario, this nonlinearity-induced distortion is deterministic and may be mitigated at \ac{TX} or \ac{RX}. On the downside, as will be shown later, one is either forced to take into account the Kerr-nonlinearity-induced spectral broadening and, thus, use a wider bandwidth compared to the symbol rate \cite{yousefi_per-sample_2011}; or, operate in a regime where spectral broadening can be neglected \cite{kaminow_chapter_2002}. The first approach reduces \ac{SE}, whereas the second limits the design and hardware options, e.g., with respect to the symbol rate.

In this work, we consider \ac{DSP} algorithms that have shown to outperform physical methods such as optical phase conjugation \cite{pepper_compensation_1980}, or optical back propagation \cite{bidaki_raman-pumped_2020}. Those digital approaches can be further divided into three types, \emph{(i)} a static, analytical, and conventional equalization by fixed algorithms, such as the Volterra-series \cite{peddanarappagari_volterra_1997}, \ac{DBP} \cite{li_electronic_2008}, and perturbation models \cite{mecozzi_nonlinear_2012} (a good overview about those can be found in \cite{cartledge_digital_2017}); \emph{(ii)} \ac{NFT}-based schemes \cite{yousefi_information_2014, yousefi_information_2014-1, yousefi_information_2014-2}; or \emph{(iii)} \ac{DL} techniques with architectural templates based on the aforementioned conventional systems -- or purely based on, e.g., a \ac{NN} \cite{karanov_end--end_2018}.

% What is the difference to our last publication?
This paper reports significant progress over \cite{uhlemann_deep-learning_2020}, where a so-called \ac{AE} with a linear \ac{TX} was trained to mitigate nonlinear distortions in a regime where spectral broadening is significant. The training results have shown that the \ac{AE} is not fully able to compensate for the aforementioned nonlinear impairments at higher input powers $P>5\,\mathrm{dBm}$. In this paper, we extend the \ac{AE} of \cite{uhlemann_deep-learning_2020} to include a \ac{NLC} architecture, effectively implementing a nonlinear \ac{TX}. Note that the linear \ac{TX} of \cite{uhlemann_deep-learning_2020} is still contained within the new model as a special case, allowing simple evaluation of the additional gains.

% What inspired the new solution?
The nonlinear extension is inspired by the so-called split \ac{DBP} consisting of a nonlinear and joint mitigation at \ac{TX} and \ac{RX}, providing the best equalization performance \cite{lavery_benefit_2016}.

% Forecast of the obtained results and insights.
As will be shown later, this newly introduced nonlinearity at the \ac{TX} allows to operate at higher input powers when compared to the linear \ac{AE} or conventional systems. One particularity is that training the proposed structure requires a specific procedure that we refer to as ``$\gamma$-lifting'' to achieve stable convergence, and to find better local optima.

% Comparison with related publications.
\ac{DL}-techniques are already widely used in almost all parts of an optical communication system. The novelty of this paper is the application of an architectural template with nonlinear \ac{TX}, i.e., its pulseshaping, as well as its particular training method.

% Häger
In a similar spirit, e.g., Häger et al. \cite{hager_physics-based_2021}, proposed a trainable \ac{SSFM}, or \ac{DBP}, at the \ac{RX} of which the first half of the compensating path may be moved to the \ac{TX} and used as \ac{PD}. Despite the fact that our trainable architectural template is not based on the \ac{SSFM}, we train the \ac{PD} directly as part of the \ac{TX}. This allows the \ac{TX} to learn the opportunities of a \ac{PD} seeing all subsequent components. 

% Neskorniuk
Neskorniuk et al.  \cite{neskorniuk_end--end_2021} have used a trainable nonlinear \ac{PD} based on cubic correction terms over an approximated channel model applying the perturbation method. There, they have shown that the training can be significantly stabilized and accelerated up to a specific input power. However, we operate at input powers where this alternative channel model differs too much from the more accurate \ac{SSFM}, which we have applied in this work. Further, we also included the quasi-analog pulseshaping into the training.

% Gaiarin
Gaiarin et al. \cite{span_time-bandwidth_2019} have trained a transmitter based on the \ac{NFT} \cite{gaiarin_end--end_2021}, providing another nonlinear \ac{TX} structure. Yet, it has been shown that \ac{NFT}-based systems are currently far from spectrally efficient operations.

The remainder of this work is structured as follows. Section~\ref{sec:system} provides a short description of the channel, the considered classic split \ac{DBP}, as well as its performance drop at high launch powers.
In section~\ref{sec:autoencoder} the architectural template of the \ac{AE} is introduced including the nonlinear \ac{TX}. The performance obtained by a conventional training is presented in section~\ref{sec:training}. Section~\ref{sec:gamma-lifting} proposes a new training procedure tailored to the opticel fiber channel that leads to improved equalization capabilities of the \ac{AE}. Finally, section~\ref{sec:summary} renders some conclusions and provides an outlook to future extensions.

\begin{table}[b] % Channel parameters
	\caption{Simulation parameters}
	\begin{center}
		\begin{tabular}{c|c|c}
			%\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
			%\hline
			\textbf{Property}&\textbf{Symbol}&\textbf{Value} \\
			\hline
			%\cline{2-4} 
			%\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
			Planck's constant&$h$&$6.626\cdot 10^{-34}\,\si{\joule\second}$ \\
			Carrier frequency&$f_0$&$193.55\,\si{\tera\hertz}$ \\
			Attenuation&$\alpha$&$0.046\,\si{\per\kilo\meter} \mathrel{\widehat{=}} 0.2\, \mathrm{dB}\,\mathrm{km}^{-1}$ \\
			Chromatic dispersion&$\beta_2$&$-21.67\,\si{\pico\second\squared\per\kilo\meter}$ \\
			Kerr-nonlinearity&$\gamma$&$1.27\,\si{\per\kilo\meter\per\watt}$ \\
			Spontaneous emission&$n_\mathrm{sp}$&$1$ \\
			Fiber length&$\ell$&$1000\,\si{\kilo\meter}$ \\
			Simulation sampling rate&$f_\mathrm{sim}$&$1\,\si{\tera\hertz}$ \\
			No. of SSFM-steps&$N_\mathrm{SSFM}$&$ 200 $ \\
			Launch power&$P$&$\left\{-30\,\mathrm{dBm}, \,\ldots,\,10\,\mathrm{dBm}\right\}$ \\
			Bandwidth of TX/RX&$B_\mathrm{w}$&$20\,\si{\giga\hertz}$ \\
			%\hline
			%copy& More table copy$^{\mathrm{a}}$& &  \\
			%\hline
			%\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
		\end{tabular}
		\label{tab:channel-parameters}
	\end{center}
\end{table}


\section{System model and performance references}\label{sec:system}\acresetall 

As the challenge of spectral broadening shall stay the same compared to \cite{uhlemann_deep-learning_2020} we use the same channel model comprising the band-limited \ac{DAC} (represented by a \ac{LPF}), the optical fiber, and a band-limited \ac{ADC}, i.e., again an \ac{LPF} as shown in the dashed gray box of Fig.~\ref{fig:system}. This model not only holds for the reference system but also for the \ac{AE} as introduced later.

The optical fiber is simulated via the symmetric \ac{SSFM} following the Wiener-Hammerstein model and, thus, approximating a solution of the \ac{NLSE} \cite{agrawal_nonlinear_2000}
\begin{equation}
	\frac{\partial q(t,z)}{\partial z}= j\frac{\beta_2}{2}\frac{\partial^2 q(t,z)}{\partial t^2}-j\gamma |q(t,z)|^2 q(t,z) + n(t,z),
	\label{eq:nlse}
\end{equation}
where ideal Raman amplification is assumed and, hence, the term accounting for fiber attenuation $\alpha$ was removed. Here $q(t,z)$ is the optical baseband signal with time $t$ and distance $z$. Alongside mitigating the attenuation, the amplification introduces noise $n(t,\,z)$ with power spectral density
\begin{equation}
	\rho_\mathrm{n} = n_\mathrm{sp} h f_0 \alpha.
\end{equation}
The corresponding channel parameters are summarized in Tab.~\ref{tab:channel-parameters}. As we consider a single channel and single polarization system the only observable manifestation of the \mbox{Kerr-effect} is \ac{SPM}.

Among the fiber parameters, also some of the signal processing, e.g., those of the converters or \acp{DSP}, are fixed to obtain comparable systems; e.g., the supported bandwidth of both converters is set to $B_\mathrm{w}=20\,\mathrm{GHz}$. To avoid artificially limiting the \ac{SE} we have chosen a symbol rate of $R_\mathrm{s}=B_\mathrm{w}=20\,\mathrm{GBd}$ and hence, a symbol duration of $T=1/R_\mathrm{s}=50\,\mathrm{ps}$. The simulation bandwidth is $f_\mathrm{sim}=1\,\mathrm{THz}$ such that one obtains $f_\mathrm{sim}R_\mathrm{s}^{-1}=50$ samples per symbol. The resulting \ac{TBP} is $\Pi_\mathrm{TB}=T\cdot B_\mathrm{w}=1$.

The alphabet, or set of message symbol indices, is $\mathcal{M}=\left\{0,\,\ldots,\,M-1\right\}$ with $M=256$ and the number of transmitted symbols is $N_\mathrm{B}$.

As performance measure, we use the \acf{SE} defined as
\begin{equation}
	\eta=\frac{I\left(s;\,\widehat{s}\right)}{T \cdot B_\mathrm{w}}=\frac{I\left(s;\,\widehat{s}\right)}{\Pi_\mathrm{TB}}\stackrel{\Pi_\mathrm{TB}=1}{=}I\left(s;\,\widehat{s}\right),
\end{equation}
where $I(s;\,\widehat{s})$ is the mutual information between the distributions of the transmitted $s$ and the received (hard decided) symbol indices $\widehat{s}$ as shown in Fig.~\ref{fig:system}  (compare to \cite{uhlemann_deep-learning_2020}).

Here we use histograms of hard decided symbols at \ac{RX} to easily include the whole \ac{RX}-\ac{DSP} in the chosen performance measure. Obviously, the performance could be improved by using soft outputs. But, in this work, we are more interested in studying how to mitigate the drop of \ac{MI} at high launch power and how to address this by means of pulse shaping.


\subsection{Spectral broadening revisited}

Taking into account the considered power range for $P$, we obtain a dispersion length of
\begin{equation}
	\ell_\mathrm{D}=T^2/|\beta_2|=115\,\mathrm{km}
\end{equation}
and a nonlinear length of
\begin{equation}
	\ell_\mathrm{NL}(P)=1/(\gamma P)\in \left[78,\,78\cdot 10^{4}\right]\,\mathrm{km}
\end{equation}
such that $\ell_\mathrm{D} < \ell_\mathrm{NL}$ does not always hold \cite{agrawal_nonlinear_2000}. This way we operate in a regime where spectral broadening cannot be neglected \cite{essiambre_capacity_2010}. Further it holds that
\begin{equation}
	\ell_\mathrm{NL}(P)<\ell\ \forall\ P>-1.0\,\mathrm{dBm}.
	\label{eq:nonlinear-length}
\end{equation}
Consequently, th received signal's bandwidth definitely exceeds the supported system bandwidth $B_\mathrm{w}=R_\mathrm{s}$ for conventional communication systems (and their corresponding equalization) as there is no margin implemented between $B_\mathrm{w}$ and the original signal bandwidth $R_\mathrm{s}$.\footnote{Note that a margin would artificially increase the \ac{TBP} and, hence, lower the \ac{SE}.} Next, we specify the goal for the \ac{AE} more precisely to ``Learning a high \ac{MI} despite the effect of spectral broadening.''

%\begin{figure}[t] % Comparison of DBP at RX and TX
%	\centering
%	\begin{tikzpicture}[scale=1.0, spy using outlines={rectangle, black, magnification=2, size=1cm, connect spies}]
%		\begin{axis}[width=1.0\columnwidth,
%			height=20em,
%			font=\small,
%			legend cell align={left},
%			legend style={font=\small, fill opacity=0.8, text opacity=1.0, at={(0.5,-0.2)}, anchor=north},
%			legend columns=1,
%			axis line style = thick,
%			%xtick={-30.0, -25.0, ..., 10.0},
%			%yticklabels={0.0, ..., 10.0},
%			xlabel={Input power $P$ in (dBm)},
%			ylabel={Spectral efficiency $\eta$ in $\left(\frac{\mathrm{bit}}{\mathrm{s\cdot Hz}}\right)$},
%			grid=major,
%			xlabel near ticks,
%			ylabel near ticks,
%			xmin=-30.0,   xmax=10,
%			ymin=0,   ymax=9,
%			nodes near coords={
%				%\tiny \pgfmathprintnumber[precision=3]{\pgfplotspointmeta}
%			},]
%			\addplot [black, mark=none, dashed] coordinates {(-30, 8) (10, 8)};
%			\node[above] at (axis cs:-22, 8) {\small{$M_\mathrm{b}=8\,\mathrm{\frac{bit}{symbol}}$}};
%			
%			% Shannon limit
%			\addplot[very thick, color=black, mark=|, mark size=4pt, mark repeat=1, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y index = 326, col sep=semicolon] {\results 20211119160424/evaluation_20211119160424.csv};
%			
%			% Constellation constrained capacity (256-QAM) with hard decisions
%			\addplot[very thick, color=gray, mark=square, mark size=4pt, mark repeat=2, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y index = 328, col sep=semicolon] {\results 20211119160424/evaluation_20211119160424.csv};
%			
%			% Classic DBP TRX ADC
%			\addplot[very thick, color=red, mark=none, mark size=4pt, mark repeat=2, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y index = 328, col sep=semicolon] {\results 20211119152924/evaluation_20211119152924.csv};
%			
%			% Classic DBP-TX ADC 
%			\addplot[thick, color=blue, mark=o, mark size=4pt, mark repeat=2, mark phase=0] table [x expr=10*log10(\thisrowno{35}*1000), y index = 330, col sep=semicolon] {\results 20211119144254/evaluation_20211119144254.csv};
%			
%			\addplot[thick, color=cyan, mark=o, mark size=4pt, mark repeat=2, mark phase=0] table [x expr=10*log10(\thisrowno{35}*1000), y index = 330, col sep=semicolon] {\results 20211119133948/evaluation_20211119133948.csv};
%			
%			% Classic DBP-RX ADC
%			\addplot[thick, color=green, mark=o, mark size=4pt, mark repeat=2, mark phase=0] table [x expr=10*log10(\thisrowno{34}*1000), y index = 329, col sep=semicolon] {\results 20211119130834/evaluation_20211119130834.csv};
%			
%			% Gray background
%			\begin{pgfonlayer}{background}
%				\draw[fill=black!10] (axis cs:-30, 0) rectangle (axis cs:-10, 9);
%			\end{pgfonlayer}
%			
%			\legend{,
%				{Upper bound $C_\mathrm{Sh}$ \cite{kramer_upper_2015}},
%				%{Constellation constrained cap. $C_\mathrm{CC}$ (uniform 256-QAM)},
%				{Max. MI after hard decision $I_\mathrm{CC}$ (256-QAM)},
%				{Split DBP w/ Power Normalization},
%				{DBP as PD w/o Power Normalization},
%				{DBP as PD w/ Power Normalization},
%				{DBP as PE},
%			}
%		\coordinate (spypoint) at (axis cs:-2,7.5) {}; 
%		\coordinate (spyviewer) at (axis cs:-10,2.5) {}; 
%		%\spy[width=3cm,height=2cm] on (spypoint) in node [fill=white] at (spyviewer); 
%		\end{axis}
%	\end{tikzpicture}
%	\caption{Performance evaluation and comparison of all three conventional systems based on \ac{DBP}. The \ac{SE} $\eta$ over input power $P$ for the different locations of the \ac{DBP}-equalizer (\ac{PD} at \ac{TX}, \ac{PE} at \ac{RX}, and both) is shown. The performance of \ac{PD} and \ac{PE} are almost same, whereas the split version shows a minor advantage.}
%	\label{fig:dbp-tx-rx-comparison}
%\end{figure}

\begin{figure}[t] % Impact of LPF on DBP at RX
	\centering
	\begin{tikzpicture}[scale=1.0, spy using outlines={rectangle, black, magnification=1.5, size=1.2cm, connect spies}]
		\begin{axis}[title={}, 
			width=1.0\columnwidth,
			height=22em,
			font=\small,
			legend cell align={left},
			%legend style={font=\small, fill opacity=0.8, text opacity=1.0, at={(0.5,-0.2)}, anchor=north},
			legend style={font=\small, fill opacity=0.9, text opacity=1.0,},
			legend columns=1,
			legend pos=south west,
			axis line style = thick,
			%xtick={-30.0, -25.0, ..., 10.0},
			%ytick={0.0, 2.0, 4.0, ..., 12.0},
			xlabel={Input power $P$ in (dBm)},
			ylabel={Spectral efficiency $\eta$ in $\left(\frac{\mathrm{bit}}{\mathrm{s\cdot Hz}}\right)$},
			grid=major,
			xlabel near ticks,
			ylabel near ticks,
			xmin=-30.0,   xmax=10,
			ymin=0,   ymax=9,
			nodes near coords={
				%\tiny \pgfmathprintnumber[precision=3]{\pgfplotspointmeta}
			},]
		
			% Gray background
			\begin{pgfonlayer}{background}
				\draw[fill=black!10] (axis cs:-30, 0) rectangle (axis cs:-10, 9);
			\end{pgfonlayer}
		
			\addplot [very thick, forget plot, black, mark=none, dashed] coordinates {(-30, 8) (10, 8)};
			\node[above] at (axis cs:-24, 8) {\small{$M_\mathrm{b}=8\,\mathrm{\frac{bit}{symbol}}$}};
			
			% Shannon limit
			\addplot[very thick, color=black, mark=|, mark size=4pt, mark repeat=1, mark phase=0, name path=SHANNON] table [x expr=10*log10(\thisrowno{33}*1000), y index = 326, col sep=semicolon] {\results 20211119160424/evaluation_20211119160424.csv};
			\addlegendentry{{Upper bound $C_\mathrm{Sh}$ \cite{kramer_upper_2015}}};
			
			\addplot[draw=none, forget plot, mark=none, dashed, name path=INF] coordinates {(-30, 10) (10, 10)};
			\addplot[forget plot, black!30] fill between [of=INF and SHANNON];
			\node[above, align=center] at (axis cs:-24, 6.3) {Unattainable\\region};
			
			% Constellation constrained capacity (256-QAM) with hard decisions
			\addplot[very thick, color=gray, mark=o, mark size=4pt, mark repeat=2, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y index = 328, col sep=semicolon] {\results 20211119160424/evaluation_20211119160424.csv};
			\addlegendentry{{Max. MI $I_\mathrm{CC}$ (256-QAM)}};
			
			\addplot[forget plot, draw=none, name path=A, no markers, mark options={decoration={name=none}}, decoration={text along path,
				text={{without LPF}},raise=+8pt,
				text align={left indent={0.76\dimexpr\pgfdecoratedpathlength\relax}},
			},
			postaction={decorate}] table [x expr=10*log10(\thisrowno{33}*1000), y index = 328, col sep=semicolon] {\results 20211119160424/evaluation_20211119160424.csv};
			
			\addlegendimage{empty legend}
			\addlegendentry{\hspace{-.7cm}\textbf{Split DBP {\color{red}without LPF}:}};
			
			% Classic DBP-RX
			%\addplot[very thick, color=violet, mark=none, mark size=4pt, mark repeat=1, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y index = 327, col sep=semicolon] {\evaluation{20211217150203}{20211217150203}};
			%\addplot[very thick, color=orange, mark=none, mark size=4pt, mark repeat=1, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y index = 327, col sep=semicolon] {\evaluation{20211217130947}{20211217130947}};
			\addplot[very thick, color=green!40!black, mark=none, mark size=4pt, mark repeat=1, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y index = 327, col sep=semicolon] {\evaluation{20211217114913}{20211217114913}};			
			\addlegendentry{{$N_\mathrm{SSFM}=600$}};	
			
			\addplot[very thick, color=green!60!black, mark=none, mark size=4pt, mark repeat=1, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y index = 327, col sep=semicolon] {\evaluation{20211217103444}{20211217103444}};
			\addlegendentry{{$N_\mathrm{SSFM}=400$}};
			
			\addplot[very thick, color=green!80!black, mark=none, mark size=4pt, mark repeat=1, mark phase=0, name path=HIGH] table [x expr=10*log10(\thisrowno{33}*1000), y index = 327, col sep=semicolon] {\evaluation{20211217095804}{20211217095804}};
			\addlegendentry{{$N_\mathrm{SSFM}=200$}};
			
			% Classic DBP TRX with ADC
			
			\addlegendimage{empty legend}
			\addlegendentry{\hspace{-.7cm}\textbf{Split DBP with LPF:}};
		
			\addplot[very thick, color=blue, mark=none, mark size=4pt, mark repeat=2, mark phase=0, name path=LOW] table [x expr=10*log10(\thisrowno{33}*1000), y index = 328, col sep=semicolon] {\results 20211119152924/evaluation_20211119152924.csv};
			\addlegendentry{{$N_\mathrm{SSFM}=200$}};
			
			\addplot[forget plot, yellow!30] fill between [of=HIGH and LOW];
			
			\addplot[forget plot, draw=none, name path=A, no markers, mark options={decoration={name=none}}, decoration={text along path,
				text={{with LPF}},raise=+4pt,
				text align={left indent={0.7\dimexpr\pgfdecoratedpathlength\relax}},
			},
			postaction={decorate}] table [x expr=10*log10(\thisrowno{33}*1000), y index = 328, col sep=semicolon] {\results 20211119152924/evaluation_20211119152924.csv};
		
			\coordinate (spypoint) at (axis cs:7.4,7.8) {}; 
			\coordinate (spyviewer) at (axis cs:-9,4.0) {}; 
			%\spy[width=2cm,height=1.5cm] on (spypoint) in node [fill=white] at (spyviewer); 
		\end{axis}
	\end{tikzpicture}
	\caption{Comparison of the performance of a split \ac{DBP} with and without (DAC/ADC-induced) \acp{LPF}. The numerical accuracy is sufficient such that it is the \acp{LPF} that limit performance.}
	\label{fig:dbp-reference}
\end{figure}

\begin{figure*}[ht] % AE CNN
\begin{subfigure}[c]{\textwidth}
	\centering
	\includesvg[width=\textwidth, inkscapearea=page]{aecnn-tx}
	\subcaption{}
	\label{fig:aecnn-tx}
	\vspace{1em}
\end{subfigure}
\begin{subfigure}[c]{\textwidth}
	\centering
	\includesvg[width=0.7\textwidth, inkscapearea=page]{aect-rx}
	\subcaption{}
	\label{fig:aecnn-rx-i}
	\vspace{1em}
\end{subfigure}
\begin{subfigure}[c]{\textwidth}
	\centering
	\includesvg[width=0.7\textwidth, inkscapearea=page]{aecnn-rx}
	\subcaption{}
	\label{fig:aecnn-rx-ii}
	\vspace{1em}
\end{subfigure}
\caption{Architectural template of the proposed \ac{AE} implementing the \ac{TX} and \ac{RX}-\ac{DSP}. Trainable blocks are colored in yellow. (\subref{fig:aecnn-tx}) shows the \ac{CNN}-based \ac{TX}-template, (\subref{fig:aecnn-rx-i}) depicts \ac{RX} Option 1 as used in \cite{uhlemann_deep-learning_2020}, and (\subref{fig:aecnn-rx-ii}) is \ac{RX} Option 2 as introduced in this work.}
\label{fig:aecnn}
\end{figure*}

\subsection{Limitations of Digital Back Propagation}

We consider three different reference systems with \ac{NLC}. First, a \ac{PD}-only mitigation at \ac{TX}, second a \ac{PE}-only at \ac{RX}, and third, a joint version. Thereby, all three reference systems are covered by Fig.~\ref{fig:dbp-tx} for their \ac{TX} and Fig.~\ref{fig:dbp-rx} for their \ac{RX}. 

As shown, the \acp{TX} share a conventional 256-\ac{QAM} that translates the symbol indices $\mathbf{s}\in\mathcal{M}^{N_\mathrm{B}}$ to complex constellation symbols $\mathbf{c}\in\mathbb{C}^{N_\mathrm{B}}$. An ideal Nyquist pulse-shaping (consisting of an upsampling to simulation frequency $f_\mathrm{sim}$ and a raised cosine pulse shaping with roll-off $\beta_\mathrm{R}=0$) lead to the bare transmit signal $\Tilde{\mathbf{x}}$. 
Typically a two-fold oversampling is used, whereas we use an oversampling of $u_\mathrm{sam}={f_\mathrm{sim}}/{R_\mathrm{s}}=50$ for a fair comparison with the later introduced trainable models that shall not learn to compensate any inaccuracy, and to exclude a numerical mismatch between channel and equalizer.
It follows an \ac{NLC} as \ac{PD} that is realized by a \ac{DBP}, which compensates for a fiber length of either $\ell_\mathrm{DBP}=\ell$ for \ac{PD}-only \cite{essiambre_fibre_2005} or $\ell_\mathrm{DBP}=\frac{\ell}{2}$ for joint mitigation (also called ``split \ac{NLC}'' or ``split \ac{DBP}'') \cite{lavery_benefit_2016}. For a \ac{PE}-only mitigation this block is skipped. A subsequent \ac{LPF} plus power normalization generate the transmit signal $\mathbf{x}$.

The \ac{RX} of a \ac{PE}-only and joint mitigation starts with a \ac{DBP} processing of the received signal $\mathbf{y}$ at simulation rate, which is already lowpass-filtered by the channel (see converters in Fig.~\ref{fig:system})\footnote{In the simulation the \ac{ADC} belongs to the channel, but technically the channel does not filter the signal.}. For a \ac{PD}-only mitigation this block is not present. An \ac{LPF} assures a correct downsampling to symbol rate $R_\mathrm{s}$ for a subsequent minimum distance demapping.
 
All aforementioned \ac{DBP} algorithms are based on the symmetric \ac{SSFM} following the Wiener-Hammerstein model as shown in \cite{millar_mitigation_2010} that is also used for the channel simulation. In the following, we refer to all three conventional algorithms as \ac{DBP} and only distinguish with respect to their location (\ac{TX}, \ac{RX}, and ``split'').

It can be shown that the performance in terms of \ac{SE} is almost equivalent for both the \ac{DBP} at \ac{RX} as well as \ac{TX}. Here, as ideal Raman amplification is assumed, there should be no change in power by the \ac{PD}. The split \ac{DBP} shows a minor performance gain compared to a single \ac{PD} or \ac{PE} \cite{lavery_benefit_2016}.

Fig.~\ref{fig:dbp-reference} shows the performance of the split \ac{DBP} (blue) and compares it with \emph{(i)} an upper bound proposed by Kramer et al. \cite{kramer_upper_2015} that is equivalent to the Shannon limit and \emph{(ii)} the constellation constrained mutual information $I_\mathrm{CC}$ for an \ac{AWGN} channel based on hard decisions and assuming a 256-QAM. The latter curve is not a bound for optical communications but only indicates that, for low input powers, the conventional systems achieve an almost optimal equalization. For high input powers, $I_\mathrm{CC}$ saturates as expected due to the constrained constellation.

It was already shown that for a \ac{PD}-only implementation ``\ac{SPM} can be eliminated, within experimental error, up to where the transmitter bandwidth limits are reached'' \cite{roberts_electronic_2006}. Hence, in general the chosen \ac{PD} leads to a transmit signal that occupies more bandwidth than the supported one by the converters. The same holds for the application of a \ac{PE}-only where now the receiver bandwidth limits the resulting performance. Hence, to overcome spectral broadening introduced by Kerr-nonlinearity, one has to take into account an artificial bandwidth expansion. This expansion combined with the \ac{LPF} explains the performance drop of the split \ac{DBP} at high launch powers.

To confirm this, Fig.~\ref{fig:dbp-reference} additionally shows the \ac{SE} of the split \ac{DBP} without the aforementioned \acp{LPF} (green). Indeed, removing the \ac{LPF} leads to the expected near optimal performance that may be achievable by completely compensating for the band limitation. Nevertheless, there is still a drop that can be related to the limited accuracy of the \ac{SSFM}, i.e., the number of steps $N_\mathrm{SSFM}$ used for the channel and the \ac{DBP}. This numerical issue is beyond the limitation of the \ac{LPF}, and thus, of no further concern. Moreover, all performance losses observed in our simulation and training setup can be attributed to the combination of spectral broadening and lowpass filtering, and not to numerical inaccuracies of the \ac{SSFM}.

\subsection{Discussion of Conventional Reference Curves}

Hence, even if the \ac{DBP} currently shows the best mitigation performance, and indeed compensates for the nonlinear impairments almost perfectly, this only holds for the case where \ac{DAC}, and/or \ac{ADC} support a significantly larger bandwidth than would be required by the actual message information, at the expanse of \ac{SE}.

This gives rise to the assumption that better solutions than \ac{DBP} in terms of \ac{SE} exist for the case where both converters significantly limit the bandwidth. I.e., the goal is to enter the attainable region between the curves with and without \ac{LPF}, indicated in yellow in Fig.~\ref{fig:dbp-reference}. While this goal has not changed since \cite{uhlemann_deep-learning_2020}, we now can apply both an extended AE and a new training procedure to further close this gap.

\input{usr/content-tcom/autoencoder}
\input{usr/content-tcom/training}
\input{usr/content-tcom/gammalifting}
\input{usr/content-tcom/results}
\input{usr/content-tcom/summary}

==> usr/content/gamma-lifting/gammalifting.tex <==




==> usr/content/gamma-lifting/results.tex <==
% !TeX spellcheck = en_US

%\begin{figure*}[ht]
%	\newcommand{\eachnthpoint}{250}
%	\centering
%	%\tikzset{external/remake next}
%	\tikzset{switch/.code={\xdef\param{#1}}}
%	\pgfdeclareplotmark{rect}
%	{%
%		\pgfmathsetmacro\result{8*mod(\param+1,2)}
%		\fill[
%		fill=black!\result,
%		draw=none,
%		%minimum height={\y1*(\pgfkeysvalueof{/pgfplots/ymax}-\pgfkeysvalueof{/pgfplots/ymin})},
%		%width=1,
%		opacity=1] (0, \pgfkeysvalueof{/pgfplots/ymax}) rectangle (1, \pgfkeysvalueof{/pgfplots/ymin});
%	}%
%	\begin{tikzpicture}[scale=1.0, spy using outlines={rectangle, black, magnification=3, size=1cm, connect spies}]
%		\pgfplotsset{
%			xmin=0, xmax=85000,
%			width=\textwidth/1.1,
%			height=20em,
%			axis line style = thick,
%			set layers,% using layers
%			mark layer=axis background% defines the layer of the marks
%		}
%		
%		\begin{axis}[title={},
%			font=\small,
%			xlabel={Training iteration},
%			axis y line* = left,
%			%ylabel={Learning rate \pgfplotsplotfromname{pgfplots:lr} Loss $\mathcal{L}_\mathrm{CE}$ \pgfplotsplotfromname{pgfplots:loss}},
%			ymajorgrids = true,
%			ylabel near ticks,
%			xlabel near ticks,
%			%ymin=1e-6,   ymax=1e2,
%			ymin=0,   ymax=6,
%			ylabel style = {align = right},
%			ylabel = {Loss $\mathcal{L}_\mathrm{CE}$\\$\gamma$-lifted \pgfplotsplotfromname{pgfplots:loss}\\no lifting \pgfplotsplotfromname{pgfplots:loss-nogammalifting}},
%			%ymode=log
%			]	
%			% LOSS corresponding to \eta=8 ...
%			\addplot [black, mark=none, dashed] coordinates {(0, 1.91969252353157) (90000, 1.91969252353157)};
%			
%			% LOSS corresponding to \eta=5.4 ...
%			\addplot [black, mark=none, dashed] coordinates {(0, 1.61511451948765) (90000, 1.61511451948765)};
%			
%			% BACKGROUND INDICATORS
%			%\addplot[ scatter,only marks,mark=rect, visualization depends on={\thisrowno{1} \as \runid}, scatter/@pre marker code/.append style= {/tikz/switch=\runid}, each nth point=\eachnthpoint, filter discard warning=false, unbounded coords=discard,] table [col sep=semicolon, x expr=\coordindex, y expr=1]{\results 20211117102456/training_20211117102456_history.csv};	
%			
%			% LOSS		
%			\addplot[very thick, color=green!70!black] table [col sep=semicolon, x expr=\coordindex, y expr=(\thisrowno{2}), each nth point=\eachnthpoint, filter discard warning=false, unbounded coords=discard] {%
%				\results 20211118075434/training_20211118075434_history.csv%
%			}; 
%			\label{pgfplots:loss-nogammalifting}		
%			
%			% LOSS gamma lifted	
%			\addplot[very thick, color=green] table [col sep=semicolon, x expr=\coordindex, y expr=(\thisrowno{2}), each nth point=\eachnthpoint, filter discard warning=false, unbounded coords=discard] {%
%				\results 20211117102456/training_20211117102456_history.csv%
%			}; 
%			\label{pgfplots:loss}		
%			
%			% LOSS gamma lifted	
%			\addplot[very thick, color=blue] table [col sep=semicolon, x expr=\coordindex, y expr=(\thisrowno{3}), each nth point=\eachnthpoint, filter discard warning=false, unbounded coords=discard] {%
%				\results 20211122132228/training_20211122132228_history.csv%
%			}; 
%			\label{pgfplots:loss-noiselifting}
%			
%			% LEARNING RATE
%			%\addplot[very thick, color=magenta] table [col sep=semicolon, x expr=\coordindex, y expr=(\thisrowno{6}), each nth point=\eachnthpoint, filter discard warning=false, unbounded coords=discard] {\results 20211117102456/training_20211117102456_history.csv};
%			%\label{pgfplots:lr}
%			
%			% TEXT NODES
%			\node[above] at (axis cs:20000, 1.91969252353157) {\small{Final loss without gamma lifting}};
%			\node[below] at (axis cs:20000, 1.61511451948765) {\small{Final $\gamma$-lifted loss}};
%		\end{axis}
%		
%		\begin{axis}[
%			title={}, 
%			font=\small,
%			axis y line*=right,
%			ylabel near ticks,
%			axis x line=none,
%			ymin=0,   ymax=1.5,
%			ylabel style = {align = right},
%			ylabel={Kerr-NL $\gamma$ in $\left(\mathrm{km}^{-1}\,\mathrm{W}^{-1}\right)$}\\$\gamma$-lifted \pgfplotsplotfromname{pgfplots:gamma}\\no lifting \pgfplotsplotfromname{pgfplots:gamma-nogammalifting},
%			]
%			
%			% GAMMA
%			\addplot[very thick, color=magenta!70!black] table [col sep=semicolon, x expr=\coordindex, y expr=(\thisrowno{3}), each nth point=\eachnthpoint, filter discard warning=false, unbounded coords=discard] {\results 20211118075434/training_20211118075434_history.csv}; 
%			\label{pgfplots:gamma-nogammalifting}
%			
%			% GAMMA gamma lifted
%			\addplot[very thick, color=magenta] table [col sep=semicolon, x expr=\coordindex, y expr=(\thisrowno{3}), each nth point=\eachnthpoint, filter discard warning=false, unbounded coords=discard] {\results 20211117102456/training_20211117102456_history.csv}; 
%			\label{pgfplots:gamma}	
%		\end{axis}
%	\end{tikzpicture}
%	\caption{Loss over training iteration or epoch with and without $\gamma$-lifting. The lower the loss, the higher the resulting spectral efficiency.}
%	\label{fig:loss-over-iteration}
%\end{figure*}

%\begin{figure}
%\centering
%\begin{tikzpicture}[scale=1.0, spy using outlines={rectangle, black, magnification=3, size=1cm, connect spies}]
%	\begin{axis}[title={}, 
%		width=\columnwidth/1.0,
%		height=20em,
%		font=\small,
%		legend cell align={left},
%		legend style={font=\small, fill opacity=0.8, text opacity=1.0, at={(0.5,-0.2)}, anchor=north},
%		legend columns=1,
%		axis line style = thick,
%		xtick={-5.0, 0.0, ..., 10.0},
%		%ytick={0.0, 2.0, 4.0, ..., 12.0},
%		xlabel={Input power $P$ in (dBm)},
%		ylabel={Estimated bit error rate},
%		grid=major,
%		xlabel near ticks,
%		ylabel near ticks,
%		xmin=-30, xmax=10,
%		ymin=0.00001,   ymax=1,
%		ymode=log,
%		nodes near coords={
%			\tiny \pgfmathprintnumber[precision=3]{\pgfplotspointmeta}
%		},]
%		\addplot [black, mark=none, dashed] coordinates {(-30, 0.003) (10, 0.003)};
%		\node[below] at (axis cs:8.8, 0.003) {\small{FEC-Threshold}};
%		
%		% Shannon limit
%		%\addplot[color=black, ultra thick] table [x expr=10*log10(\thisrowno{30}*1000), y index = 91] {\classicawgnse};
%		%\addplot[color=gray, mark=o, mark size=4pt, ultra thick] table [x expr=10*log10(\thisrowno{30}*1000), y index = 93] {\classicawgnse};
%		
%		% DBP reference
%		\addplot[very thick, color=red, mark=none, mark size=4pt, mark repeat=2, mark phase=0] table [x expr=10*log10(\thisrowno{33}*1000), y expr = \thisrowno{326}, col sep=semicolon] {\results 20211119152924/evaluation_20211119152924.csv};
%		
%		% AECT Leipzig
%		%\addplot[dashed, color=mittelblau, mark=o, mark size=4pt, mark repeat=1, mark phase=0, very thick] table [x index = 0, y expr = \thisrowno{1}/8] {\aecdnltwentyse};
%		
%		
%		% AECT
%		\addplot[very thick, color=mittelblau, mark=o, mark size=4pt, mark repeat=1, mark phase=0] table [meta index=3, x expr=10*log10(\thisrowno{33}*1000), y expr = \thisrowno{310}] {\results 20211013105616/training_20211013105616.csv};
%		
%		
%		% AECNN		
%		\addplot[very thick, color=green, mark=triangle, mark size=4pt, mark repeat=1, mark phase=0] table [col sep=semicolon, meta index=3, x expr=10*log10(\thisrowno{33}*1000), y expr=(\thisrowno{327})] {\results 20211110174947/training_20211110174947.csv};
%		
%		\legend{,
%			%{Upper bound $C_\mathrm{Sh}$ \cite{kramer_upper_2015}},
%			%{Max. MI after hard decision \ $I_\mathrm{CC}$ (uniform 256-QAM)},
%			{DBP},
%			%{AE-CT Leipzig},
%			{AE-CT Leipzig ($\gamma$-lifted)},
%			{AE-CNN ($\gamma$-lifted)},,
%		}
%	\end{axis}
%\end{tikzpicture}
%\caption{\ac{BER}-chart.}
%\label{fig:ber-chart}
%\end{figure}
